DeFiRank: Federated Pairwise Ranking for Governance in Decentralized Financial Networks

Existing governance approaches in decentralized financial networks rely on manual review processes conducted by human committees, which introduces subjective bias, creates a scalability bottleneck under high network volume, and fails to capture complex behavioural patterns and evolving network dynamics. To address these limitations, we propose \name, a federated learning-based pairwise ranking framework in which multiple institutions collaboratively train a ranking model without sharing their private transaction data. This collaborative learning enables the model to capture network-wide behavioural patterns that signify strong network participation and directly contribute to the network effect, including diversity of counterparties, usage of multiple applications, and frequency of transactions. The proposed system ranks providers based on the authenticity of their actions, promoting genuine contributors and demoting those exhibiting suspicious behaviour. We evaluate \name\ on a real-world blockchain transaction dataset. Results demonstrate that the federated approach achieves ranking performance modestly below the centralized baseline (NDCG@15: $\approx$0.87 vs.\ $\approx$0.92) while preserving data privacy and matching its ranking stability (Kendall $\tau$: $\approx$0.70 for both regimes), producing reliable governance decisions, including provider promotion and demotion (648 and 39 unique providers, respectively), without requiring centralized access to sensitive transaction data.

==> Algorithm1.tex <==
\begin{algorithm}[t]
\small
\caption{Dynamic Governance Decision Pipeline}
\label{alg:governance}
\begin{algorithmic}[1]
\REQUIRE Daily provider scores, featured-status flags, activity; baseline period $B=30$ days
\ENSURE Promotion list $\mathcal{P}$, demotion list $\mathcal{D}$
\STATE \textit{Step 1: Baseline anchors (first $B$ days)}
\STATE $\tau_{\text{promo}} \gets$ 25th percentile of active featured scores
\IF{stuck at floor (0.10)} \STATE retry at 50th percentile \ENDIF
\IF{still stuck} \STATE fall back to 75th percentile of outrank ratios \ENDIF
\STATE Clip $\tau_{\text{promo}}$ to $[0.10, 0.60]$
\STATE $K_{\text{base}} \gets$ rank with the largest score gap between featured providers \label{line:demotion_anchor}
\STATE $\rho_{\text{min}} \gets$ median outrank ratio of providers clearing $\tau_{\text{promo}}$, clipped to $[0.25, 0.70]$
\IF{$\tau_{\text{promo}}$ stuck at ceiling (0.60)} \STATE raise $\rho_{\text{min}}$ to $\geq 0.685$ \ENDIF
\medskip
\STATE \textit{Step 2: For each day}
\FOR{each day}
    \STATE Scale $\tau_{\text{promo}}$ by today's health ratio $\to$ today's threshold, clipped to $[0.10,0.60]$ \label{line:promo_threshold}
    \STATE Scale $K_{\text{base}}$ by today's size ratio $\to$ today's cutoff, clipped to $[3,150]$, capped by featured count \label{line:effective_topk}
    \STATE Drop near-inactive featured providers; skip day if fewer than 3 remain
    \STATE Flag featured providers below the cutoff for $\mathcal{D}$
    \FOR{each non-featured provider}
        \STATE Flag as candidate if its outrank fraction meets today's threshold
    \ENDFOR
\ENDFOR
\medskip
\STATE \textit{Step 3: Reliability check}
\FOR{each candidate}
    \STATE Group qualifying days into runs of consecutive dates
    \IF{a run has $\geq 2$ days and average ratio $\geq \rho_{\text{min}}$} \label{line:reliability}
        \STATE Confirm provider for $\mathcal{P}$
    \ENDIF
\ENDFOR
\RETURN $\mathcal{P}, \mathcal{D}$
\end{algorithmic}
\end{algorithm}



==> Architecture_diagram.tex <==
% architecture_diagram_twobranch_narrow.tex
% Two-branch (Provider A / Provider B side by side) version of the
% TemporalRankNet figure, re-dimensioned natively to fit ONE column
% of a two-column IEEE-style paper (columnwidth ~= 252pt ~= 8.86cm),
% rather than shrinking the original wide two-branch figure with
% \resizebox. Font sizes below are chosen for THIS width, so they
% stay legible instead of shrinking to ~4pt.
%
% Requires in the preamble of the including document:
%   \usepackage{tikz}
%   \usepackage{amsmath}
%   \usetikzlibrary{arrows.meta, calc}

\begin{tikzpicture}[
  font=\sffamily,
  >={Stealth[length=1.8mm]},
  inputbox/.style={draw, fill=blue!8, rounded corners=1pt, minimum width=0.95cm,
                    minimum height=0.85cm, font=\scriptsize, inner sep=0pt},
  lstmbox/.style={draw, thick, fill=green!15, rounded corners=4pt,
                   text width=3.4cm, align=center, minimum height=2.7cm,
                   font=\scriptsize, inner sep=2pt},
  scorerbox/.style={draw, thick, fill=orange!12, rounded corners=4pt,
                     text width=3.4cm, align=center, minimum height=2.5cm,
                     font=\scriptsize, inner sep=2pt},
  pairwisebox/.style={draw, thick, fill=red!8, rounded corners=4pt,
                        text width=7.0cm, align=center, minimum height=2.0cm,
                        font=\scriptsize, inner sep=2pt},
  outputbox/.style={draw, thick, fill=orange!12, rounded corners=4pt,
                      text width=4.6cm, align=center, minimum height=1.1cm,
                      font=\scriptsize\bfseries, inner sep=2pt},
  caption/.style={font=\tiny, align=center},
  sharedlabel/.style={font=\tiny\itshape, gray, align=center},
  scorelabel/.style={font=\scriptsize\bfseries},
  branchtitle/.style={font=\scriptsize\bfseries, align=center, text width=3.8cm},
]

% Branch centers (separation chosen so both branches + dashed border
% fit within ~8.4cm, comfortably under the 8.86cm column width)
\def\cA{2.0}
\def\cB{6.3}

%======================================================
% Titles
%======================================================
\node[branchtitle] at (\cA,16.1) {Provider $A$ \\ 7-day rolling window};
\node[branchtitle] at (\cB,16.1) {Provider $B$ \\ 7-day rolling window};

%======================================================
% Input boxes -- Provider A  (offsets symmetric around cA, pitch 0.5cm)
%======================================================
\node[inputbox] at (\cA-1.1,14.6) {$x_1^{t-6}$};
\node[font=\small] at (\cA+0.0,14.6) {$\cdots$};
\node[inputbox] at (\cA+1.1,14.6) {$x_7^{t}$};

\node[caption] at (\cA,13.95) {13 governance features\\per day, shape $(7,13)$};

%======================================================
% Input boxes -- Provider B
%======================================================
\node[inputbox] at (\cB-1.1,14.6) {$x_1^{t-6}$};
\node[font=\small] at (\cB+0.0,14.6) {$\cdots$};
\node[inputbox] at (\cB+1.1,14.6) {$x_7^{t}$};

\node[caption] at (\cB,13.95) {13 governance features\\per day, shape $(7,13)$};

%======================================================
% Dashed outer box -- TemporalRankNet
%======================================================
\node[draw, dashed, thick, rounded corners=5pt,
      minimum width=8.3cm, minimum height=8.9cm] (bigbox) at (4.15,8.85) {};
\node[font=\scriptsize\bfseries, align=center, text width=7.8cm, fill=white, inner sep=1pt] at (4.15,12.5)
      {TemporalRankNet (shared weights across $A,B$)};

%======================================================
% LSTM Encoders
%======================================================
\node[lstmbox] (lstmA) at (\cA,10.4) {
  LSTM Encoder\\[1pt]
  (2 layers, dim 64)\\[1pt]
  $(h_{t-1},c_{t-1}) \to (h_t,c_t)$\\[1pt]
  day-by-day, $t=1,\dots,7$
};
\node[lstmbox] (lstmB) at (\cB,10.4) {
  LSTM Encoder\\[1pt]
  (2 layers, dim 64)\\[1pt]
  $(h_{t-1},c_{t-1}) \to (h_t,c_t)$\\[1pt]
  day-by-day, $t=1,\dots,7$
};

\draw[<->, thick, gray] (lstmA.east) -- (lstmB.west)
      node[sharedlabel, midway, fill=white, inner sep=1pt] {shared\\weights};

\node[caption] (h7A) at (\cA,8.75) {$h_7^A$ (64-dim emb.)};
\node[caption] (h7B) at (\cB,8.75) {$h_7^B$ (64-dim emb.)};

%======================================================
% Scorers
%======================================================
\node[scorerbox] (scoreA) at (\cA,6.35) {
  Scorer\\[1pt]
  Linear$(64\to32)$ $\to$ ReLU\\[1pt]
  $\to$ Dropout$(0.1)$\\[1pt]
  $\to$ Linear$(32\to1)$
};
\node[scorerbox] (scoreB) at (\cB,6.35) {
  Scorer\\[1pt]
  Linear$(64\to32)$ $\to$ ReLU\\[1pt]
  $\to$ Dropout$(0.1)$\\[1pt]
  $\to$ Linear$(32\to1)$
};

\draw[<->, thick, gray, dashed] (scoreA.east) -- (scoreB.west)
      node[sharedlabel, midway, fill=white, inner sep=1pt] {shared\\weights};

%======================================================
% Arrows: input row -> LSTM, LSTM -> Scorer
%======================================================
\draw[->, thick] (\cA,13.6) -- (\cA,11.75);
\draw[->, thick] (\cB,13.6) -- (\cB,11.75);

\draw[->, thick] (lstmA.south) -- (scoreA.north);
\draw[->, thick] (lstmB.south) -- (scoreB.north);

%======================================================
% Score labels (bottom edge of dashed box)
%======================================================
\node[scorelabel] (sA) at (\cA,4.85) {score $s_A$};
\node[scorelabel] (sB) at (\cB,4.85) {score $s_B$};

%======================================================
% Pairwise Comparison box
%======================================================
\node[pairwisebox] (pairwise) at (4.15,3.1) {
  Pairwise Comparison\\[2pt]
  $\mathcal{L} = \mathrm{BCE}(s_A - s_B,\, y_{AB})$\\[2pt]
  $y_{AB}=1$ if $A$ outranks $B$, else $0$
};

\draw[->, thick] (sA.south) to[out=-90, in=160] (pairwise.north -| {$(pairwise.west)+(1.2,0)$});
\draw[->, thick] (sB.south) to[out=-90, in=20]  (pairwise.north -| {$(pairwise.east)-(1.2,0)$});

%======================================================
% Output box
%======================================================
\node[outputbox] (output) at (4.15,0.65) {Predicted governance\\rank ordering};

\draw[->, thick] (pairwise.south) -- (output.north);

\end{tikzpicture}
